Near-Field Beamfocusing with Polarized Antennas

One of the most relevant challenges in future 6G wireless networks is how to support a massive spatial multiplexing of a large number of user terminals. Recently, extremely large antenna arrays (ELAAs), also referred to as extra-large MIMO (XL-MIMO), have emerged as an potential enabler of this type of spatially multiplexed transmission. These massive configurations substantially increase the number of available spatial degrees of freedom (transmission modes) while also enabling to spatially focus the transmitted energy into a very small region, thanks to the properties of near-field propagation and the large number of transmitters. This work explores whether multiplexing of multiple orthogonal polarizations can enhance the system performance in the near-field. We concentrate on a simple scenario consisting of a Uniform Linear Array (ULA) and a single antenna element user equipment (UE). We demonstrate that the number of spatial degrees of freedom can be as large as 3 in the near-field of a Line of Sight (LoS) channel when both transmitter and receiver employ three orthogonal linear polarizations. In the far-field, however, the maximum number of spatial degrees of freedom tends to be only 2, due to the fact that the equivalent MIMO channel becomes rank deficient. We provide an analytical approximation to the achievable rate, which allows us to derive approximations to the optimal antenna spacing and array size that maximize the achievable rate

==> figures/room.tex <==
\begin{tikzpicture}[scale=0.50]
\begin{scope}[thick]
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(1.6,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) node (v1) {} -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(3.2,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(4.8,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(9.5,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}

\node at (5.9,3.5) {\large{$\cdots$}};

\end{scope}


\begin{scope}[shift={(0,-1.5)},thick]
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(1.6,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(3.2,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(4.8,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(9.5,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}


\end{scope}


\begin{scope}[shift={(0,-3)},thick]
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(1.6,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(3.2,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(4.8,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(9.5,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\node at (5.9,4.3) {\large{$\cdots$}};

\end{scope}




\begin{scope}[shift={(0,-5.6)},thick]
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(1.6,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(3.2,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(4.8,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(6.4,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) -- (-2.4,4.5);
\end{scope}
\begin{scope}[shift={(9.5,0)}]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) node (v2) {} -- (-2.4,4.5);
\end{scope}

\node at (5.9,4.5) {\large{$\cdots$}};

\end{scope}


\node at (0,0.1) {\large{$\vdots$}};
\node at (4,0.1) {\large{$\vdots$}};
\node at (6.9,0.1) {\large{$\vdots$}};

\node (v1) at (-0.5,4.2) {};
\node (v2) at (7.4,4.2) {};
\node (v3) at (-0.5,-1.4) {};
\node (v4) at (7.4,-1.4) {};

\draw [very thin,dotted,fill,opacity=0.1] (v1) rectangle (v4);

\draw [fill] (v1) ellipse (0.01 and 0.01);
\draw [fill]  (1.1,4.2) node (v5) {} ellipse (0.01 and 0.01);
\draw [fill]  (2.7,4.2) node (v7) {} ellipse (0.01 and 0.01);
\draw [fill]  (4.3,4.2) node (v9) {} ellipse (0.01 and 0.01);
\draw [fill]  (4.3,2.7) ellipse (0.01 and 0.01);
\draw [fill]  (2.7,2.7) ellipse (0.01 and 0.01);
\draw [fill]  (1.1,2.7) ellipse (0.01 and 0.01);
\draw [fill]  (-0.5,2.7) node (v13) {} ellipse (0.01 and 0.01);
\draw [fill]  (-0.5,-1.4) node (v17) {} ellipse (0.01 and 0.01);
\draw [fill]  (1.1,-1.4) node (v6) {} ellipse (0.01 and 0.01);
\draw [fill]  (2.7,-1.4) node (v8) {} ellipse (0.01 and 0.01);
\draw [fill]  (4.3,-1.4) node (v10) {} ellipse (0.01 and 0.01);
\draw [fill]  (7.4,-1.4) node (v12) {} ellipse (0.01 and 0.01);
\draw [fill]  (7.4,2.7) node (v14) {} ellipse (0.01 and 0.01);
\draw [fill]  (7.4,4.2) node (v11) {} ellipse (0.01 and 0.01);
\draw [fill]  (-0.5,1.2) node (v15) {} ellipse (0.01 and 0.01);
\draw [fill]  (1.1,1.2) ellipse (0.01 and 0.01);
\draw [fill]  (2.7,1.2) ellipse (0.01 and 0.01);
\draw [fill]  (4.3,1.2) ellipse (0.01 and 0.01);
\draw [fill]  (7.4,1.2) node (v16) {} ellipse (0.01 and 0.01);


\draw [dotted,thin] (v5) -- (v6);
\draw [dotted,thin] (v7) -- (v8);
\draw [dotted,thin]  (v9) -- (v10);
\draw [dotted,thin]  (v11) -- (v12);
\draw [dotted,thin]  (v13) -- (v14);
\draw [dotted,thin] (v15) -- (v16);
\draw[dotted,thin]  (v17) -- (v12);
\draw [dotted,thin]  (v1) -- (v11);
\draw [dotted,thin] (v1) -- (v17);
\draw[very thin,dotted,fill,opacity=0.1]  (3.1,-1.4) rectangle (3.9,-4);
\draw[<->,very thin] (1.1,4.8) -- (2.7,4.8);

\node at (1.9,5.1) {$\Lambda_T$}; %{$d$}; %{$\Lambda_T$};
\draw [<->,very thin] (2,-1.4) -- (2,-4);
\node at (1.6,-2.8) {$h$};
\draw [<->,very thin] (-1.4,4.2) -- (-1.4,-1.4);
\draw [<->,very thin]  (-0.5,5.5) -- (7.4,5.5);
\node at (-1.8,1.5) {$A$}; %{$(2K+1)\Lambda_T$};
\node at (3.3,5.9) {$(2K+1)\Lambda_T$};% {$B$};
\draw [->] (3.5,-4) -- (3.5,-2.9);
\draw [->] (3.5,-4)-- (4.6,-4);
\draw [->] (3.5,-4) -- (4.2,-4.7);
\node at (5,-4) {\scriptsize{$\hat{y}$}};
\node at (3.7,-2.5) {\scriptsize{$\hat{z}$}};
\node at (3.8,-5)  {\scriptsize{$\hat{x}$}};
\draw [dotted] (3.5,-4) -- (13.9,-6.2) ;
\draw [dotted] (13.9,-2) --(13.9,-6.2) ;
\draw [dotted] (13.9,-2) -- (3.5,-4);


\begin{scope}[shift={(16,-6.2)},thick]
\draw (-2.1,4.3) -- (-2.1,4.7);
\draw (-2.1,4.1) -- (-2.1,3.7);
\draw (-2,4.2) -- (-1.6,4.2);
\draw (-2.2,4.2) -- (-2.6,4.2);
\draw (-2,4.1) -- (-1.8,3.9);
\draw (-2.2,4.3) node (v2) {} -- (-2.4,4.5);
\end{scope}


\draw (4,-4.5) .. controls (4.4,-4.4) and (4.4,-4.2) .. (4.4,-4.2);
\draw (3.5,-3.3) .. controls (3.7,-3.3) and (4.1,-3.6) .. (4.0752,-3.8824);
\node at (4.1,-3.3) {$\theta$};
\node at (4.6,-4.6) {$\phi$};
%\node at (10,-2.5) {$r$};
\node at (14.6,-1) {UE};
\node at (9,4.7) {XL-MIMO};
\end{tikzpicture}
